WarPGNN: A Parametric Thermal Warpage Analysis Framework with Physics-aware Graph Neural Network

With the advent of system-in-package (SiP) chiplet-based design and heterogeneous 2.5D/3D integration, thermal-induced warpage has become a critical reliability concern. While conventional numerical approaches can deliver highly accurate results, they often incur prohibitively high computational costs, limiting their scalability for complex chiplet-package systems. In this paper, we present WarPGNN, an efficient and accurate parametric thermal warpage analysis framework powered by Graph Neural Networks (GNNs). By operating directly on graphs constructed from the floorplans, WarPGNN enables fast warpage-aware floorplan exploration and exhibits strong transferability across diverse package configurations. Our method first encodes multi-die floorplans into reduced Transitive Closure Graphs (rTCGs), then a Graph Convolution Network (GCN)-based encoder extracts hierarchical structural features, followed by a U-Net inspired decoder that reconstructs warpage maps from graph feature embeddings. Furthermore, to address the long-tailed pattern of warpage data distribution, we developed a physics-informed loss and revised a message-passing encoder based on Graph Isomorphic Network (GIN) that further enhance learning performance for extreme cases and expressiveness of graph embeddings. Numerical results show that WarPGNN achieves more than 205.91x speedup compared with the 2-D efficient FEM-based method and over 119766.64x acceleration with 3-D FEM method COMSOL, respectively, while maintaining comparable accuracy at only 1.26% full-scale normalized RMSE and 2.21% warpage value error. Compared with recent DeepONet-based model, our method achieved comparable prediction accuracy and inference speedup with 3.4x lower training time. In addition, WarPGNN demonstrates remarkable transferability on unseen datasets with up to 3.69% normalized RMSE and similar runtime.

==> figtex/Transfer_fig.tex <==
\begin{figure}[htp]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/TS_fig.pdf}
    \vspace{-10pt}
    \caption{\small Comparison of the predicted deformation map obtained from \textbf{\textit{WarPGNN}} and COMSOL on extended dataset }
    \label{fig:main_fig}
    \vspace{-15pt}
\end{figure}

==> tables/WarpageStats.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{table}[htp]
\caption{\small Statistics of Normalized Ground-Truth Warpage Values}
\vspace{-10pt}
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|cccccc}
\hline
\textbf{Bin Range}  & {[}-inf, -3{]} & {[}-3, -2{]} & {[}-2, -1{]} & {[}-1, 0{]} & {[}0, 1{]} & {[}1, 2{]} \\ \hline\hline
\textbf{Proportion} & 0.33\%         & 3.38\%       & 12.63\%      & 30.43\%     & 34.77\%    & 18.47\%    \\ \hline
\textbf{RMSE~$\downarrow$} & 0.328       & 0.190       & 0.194      & 0.126  & 0.085    & 0.054   \\ \hline
\textbf{MAE~$\downarrow$} & 0.253       & 0.144       & 0.146      & 0.097  & 0.067    & 0.041   \\ \hline
\end{tabular}
}
\label{tab:warpage_stats}
\vspace{-10pt}
\end{table}
